New Optimisation Methods for Machine Learning

A thesis submitted for the degree of Doctor of Philosophy of The Australian National University. In this work we introduce several new optimisation methods for problems in machine learning. Our algorithms broadly fall into two categories: optimisation of finite sums and of graph structured objectives. The finite sum problem is simply the minimisation of objective functions that are naturally expressed as a summation over a large number of terms, where each term has a similar or identical weight. Such objectives most often appear in machine learning in the empirical risk minimisation framework in the non-online learning setting. The second category, that of graph structured objectives, consists of objectives that result from applying maximum likelihood to Markov random field models. Unlike the finite sum case, all the non-linearity is contained within a partition function term, which does not readily decompose into a summation. For the finite sum problem, we introduce the Finito and SAGA algorithms, as well as variants of each. For graph-structured problems, we take three complementary approaches. We look at learning the parameters for a fixed structure, learning the structure independently, and learning both simultaneously. Specifically, for the combined approach, we introduce a new method for encouraging graph structures with the "scale-free" property. For the structure learning problem, we establish SHORTCUT, a O(n^{2.5}) expected time approximate structure learning method for Gaussian graphical models. For problems where the structure is known but the parameters unknown, we introduce an approximate maximum likelihood learning algorithm that is capable of learning a useful subclass of Gaussian graphical models.

==> approx-covsel/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> background-gaussian/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> background-incremental/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> colab/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> finito/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> frontmatter.tex <==
\vspace*{14cm}
\begin{center}
  \makeatletter
  \copyright\ \@author{} 2014
  \makeatother
\end{center}
\noindent
\begin{center}
  \footnotesize{~} %\aboutthesis
\end{center}
\noindent

\newpage

\vspace*{7cm}
\begin{center}
  Except where otherwise indicated, this thesis is my own original
  work.
\end{center}

\vspace*{4cm}

\hspace{8cm}\makeatletter\@author\makeatother\par
\hspace{8cm}November 12th 2014


==> inc-discus/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> saga/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:


==> submodular/macros.tex <==
%      $Id: macros.tex 506 2009-10-05 16:57:07Z daniel $    

\usepackage{booktabs}
\usepackage{relsize}
\usepackage{xspace}
\usepackage{subfig}
\usepackage{listings}
\lstloadlanguages{java}
\DeclareGraphicsRule{*}{pdf}{*}{}
\newcommand{\otoprule}{\midrule[\heavyrulewidth]}
\newcommand{\pldi}{ACM Programming Language Design and Implementation (PLDI)}
\newcommand{\taco}{ACM Transactions on Architecture and Code Optimization (TACO)}
\newcommand{\lctes}{ACM Languages, Compiler, and Tool Support for Embedded Systems (LCTES)}
\newcommand{\popl}{ACM Principles of Programming Languages (POPL)}
\newcommand{\ecoop}{European Conference for Object-Oriented Programming (ECOOP)}
\newcommand{\asplos}{ACM Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\sigmetrics}{ACM Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\oopsla}{ACM Object-Oriented Programming, Systems, Languages, and Applications (OOPSLA)}
\newcommand{\ismm}{International Symposium on Memory Management (ISMM)}
\newcommand{\veee}{ACM/USENIX Virtual Execution Environments (VEE)}
\newcommand{\micro}{ACM/IEEE International Symposium on Microarchitecture}
\newcommand{\isca}{ACM/IEEE International Symposium on Computer Architecture (ISCA)}
\newcommand{\icse}{International Conference  on Software Engineering (ICSE)}
\newcommand{\pact}{Parallel Architectures and Compilation Techniques (PACT)}
\newcommand{\casess}{ACM Compilers, Architectures, and Synthesis for Embedded Systems (CASES)}

\definecolor{tableheadcolor}{rgb}{0.8,0.8,1.0}
%\definecolor{tablealtcolor}{rgb}{0.9,0.9,1.0}
\definecolor{tablealtcolor}{rgb}{0.9,0.9,0.95}


\definecolor{todocolor}{rgb}{0.8,0.8,1.0}
\definecolor{fixcolor}{rgb}{1,0.8,0.8}
\definecolor{commentcolor}{rgb}{0.8,1.0,0.8}


\newcommand{\listingfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \begin{minipage}[t]{\textwidth-4cm}
      \lstinputlisting{#1}
    \end{minipage}
  \end{center}
  \caption{#3}#2
\end{figure}}

\newcommand{\includeabchart}[5]{
\begin{figure}[ht!]
\begin{center}
\newcommand{\atitle}{#4}
\newcommand{\btitle}{#5}
\input{charts/#1.tex}
\end{center}
\caption{#3}#2
\end{figure}}

\newcommand{\placeholderfigure}[2]{
\begin{figure}[ht!]
  \begin{center}
    \resizebox{\textwidth-2cm}{0.7\textwidth-1.4cm}{todo}
  \end{center}
  \caption{#2}#1
\end{figure}}

\newcommand{\singlegraphfigure}[3]{
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=\textwidth-2cm]{#1}
  \end{center}
  \caption{#3}#2
\end{figure}}

\usepackage[color=todocolor, colorinlistoftodos]{todonotes}

%\newcommand{\notinpart}{%
% \def\toclevel@chapter{-1}\def\toclevel@section{0}\def\toclevel@subsection{1}} \newcommand{\inpart}{
% \def\toclevel@chapter{0}\def\toclevel@section{1}\def\toclevel@subsection{2}}


%
% Stuff for pretty printing the source code using listings.sty
%


%% set Java as the default language
\lstset{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=1,
  numbersep=2em,
  language=java,                         % the language
  basicstyle=\footnotesize\ttfamily,     % the basic font family to use
  commentstyle=\itshape,                 % the font for comments
  stringstyle=\ttfamily,
%  morekeywords={@Intrinsic, @Unboxed, @RawStorage}
}
%\lstset{language=java}

\newcommand{\textjava}[1]{{\lstset{basicstyle=\ttfamily}\lstinline@#1@}}
\newcommand{\textjavafn}[1]{{\lstset{basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\usepackage{lstasm}
\usepackage{setspace}
\usepackage{ifthen}
%\usepackage{color}
%\usepackage{smallheadings}

\long\def\sfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}
%
% code
%

\newcommand{\address}{\textjava{Address}\xspace}
\newcommand{\ubregion}{\textjava{unbump-region()}\xspace}
\newcommand{\word}{\textjava{Word}\xspace}
\newcommand{\freeme}{\textjava{free()}\xspace}
\newcommand{\freemeunbump}{\textjava{unbump()}\xspace}
\newcommand{\freemeunbumpregion}{\textjava{unbump-region()}\xspace}
\newcommand{\freemeunreserve}{\textjava{unreserve()}\xspace}

%
% abbreviations
%


\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }

\newcommand{\GenMS}{\emph{GenMS}\xspace}
\newcommand{\GenImmix}{\emph{GenIX}\xspace}
\newcommand{\mmtk}{MMTk\xspace}
\newcommand{\jikes}{Jikes RVM\xspace} 
\newcommand{\jikesrvm}{\jikes} 
\newcommand{\jala}{Jalape\~{n}o\xspace} 
\newcommand{\jalapeno}{Jalape\~{n}o\xspace} 

\newcommand{\dacapo}{\textsf{DaCapo}\xspace}
\newcommand{\specjvm}{\textsf{SPECjvm98}\xspace}
\newcommand{\cattrack}{\textsf{cattrack}\xspace}
\newcommand{\spec}{\textsf{SPEC}\xspace}

\newcommand{\nurserytype}[1]{{\fontfamily{cmss}\selectfont \textsl{#1}}}
\newcommand{\alloc}{\nurserytype{allocate}\xspace}
\newcommand{\collect}{\nurserytype{collect}\xspace}
\newcommand{\redirect}{\nurserytype{redirect}\xspace}

\newcommand{\bmtype}[1]{{\textsf{#1}}}

\newcommand{\jbb}{\bmtype{jbb2000}\xspace}
\newcommand{\psjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\pjbb}{\bmtype{pjbb2005}\xspace}
\newcommand{\specjbb}{\bmtype{SPECjbb2005}\xspace}
\newcommand{\jess}{\bmtype{jess}\xspace}
\newcommand{\raytrace}{\bmtype{raytrace}\xspace}
\newcommand{\db}{\bmtype{db}\xspace}
\newcommand{\javac}{\bmtype{javac}\xspace}
\newcommand{\jack}{\bmtype{jack}\xspace}
\newcommand{\compress}{\bmtype{compress}\xspace}
\newcommand{\mpegaudio}{\bmtype{mpegaudio}\xspace}
\newcommand{\mtrt}{\bmtype{mtrt}\xspace}
\newcommand{\antlr}{\bmtype{antlr}\xspace}
\newcommand{\bloat}{\bmtype{bloat}\xspace}
\newcommand{\chart}{\bmtype{chart}\xspace}
\newcommand{\eclipse}{\bmtype{eclipse}\xspace}
\newcommand{\fop}{\bmtype{fop}\xspace}
\newcommand{\hsqldb}{\bmtype{hsqldb}\xspace}
\newcommand{\jython}{\bmtype{jython}\xspace}
\newcommand{\luindex}{\bmtype{luindex}\xspace}
\newcommand{\lusearch}{\bmtype{lusearch}\xspace}
\newcommand{\Lusearch}{\bmtype{Lusearch}\xspace}
\newcommand{\pmd}{\bmtype{pmd}\xspace}
\newcommand{\ps}{\bmtype{ps}\xspace}
\newcommand{\SPECjbb}{\bmtype{SPECjbb}\xspace}
\newcommand{\xalan}{\bmtype{xalan}\xspace}
\newcommand{\sunflow}{\bmtype{sunflow}\xspace}
\newcommand{\Sunflow}{\bmtype{Sunflow}\xspace}
\newcommand{\avrora}{\bmtype{avrora}\xspace}
\newcommand{\core}{Core2 Quad\xspace}
\newcommand{\corelong}{Intel Core2 Quad Q6600\xspace}
\newcommand{\phenom}{Phenom II\xspace}
\newcommand{\phenomlong}{AMD Phenom II X6 1055T\xspace}
\newcommand{\sandy}{i7-2600\xspace}
\newcommand{\sandylong}{Intel Core i7-2600\xspace}



\newcommand{\ghostscript}{\bmtype{ghostscript}\xspace}

\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{\nolinkurl{doi:#1}}}
%
% misc
%
\newcommand{\fix}[1]{\todo[color=fixcolor]{#1}}
\newcommand{\comment}[1]{\todo[color=commentcolor]{#1}}
\newcommand{\ifix}[1]{\todo[inline,color=fixcolor]{#1}}
\newcommand{\icomment}[1]{\todo[inline,color=commentcolor]{#1}}
\newcommand{\itodo}[1]{\todo[inline]{#1}}
\newcommand{\ignore}[1]{}
\newcommand{\mccenter}[1]{\multicolumn{1}{c|}{#1}}

%
% figure spacing
%
%\clubpenalty 10000
%\widowpenalty 10000
%\def\topfraction{0.9}
%\def\bottomfraction{0.9}
%\def\textfraction{0.1}
%\renewcommand{\singlespacing}{\renewcommand{\baselinestretch}{1.00}\small\normalsize}
%\renewcommand{\doublespacing}{\renewcommand{\baselinestretch}{1.5}\small\normalsize}
%\newcommand{\tight}{\renewcommand{\baselinestretch}{1.28}\small\normalsize}
%\renewcommand{\subfigbottomskip}{0.25ex}
%\renewcommand{\subfigcapskip}{0ex}
%\renewcommand{\subfigcapskip}{-1ex}
%\newcommand{\subfigshrink}{-0.75ex}
%\newcommand{\subfigcapspace}{2ex}

%\newcommand{\subwidth}[0]{.32\textwidth}


%
% margins
%
%\topmargin -.5truein
%\textheight 9truein
%\oddsidemargin .25truein
%\evensidemargin .25truein
%\textwidth 6truein


%
% crossreferencing footnotes
%
%\newcommand{\fnref}[1]{~(\ref{#1})}
%\newcommand{\onecolparbox}{3.1in}


%\newcommand{\textjava}[1]{{\lstset{language=java,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}
%\newcommand{\textasm}[1]{{\lstset{language=asm,basicstyle=\footnotesize\ttfamily}\lstinline@#1@}}

%%
%% Change the sections etc.
%%
%\makeatletter
%\parskip=0pt
%\renewcommand\section{\@startsection{section}{1}{\z@}%
%                                   {-2.5ex}% beforeskip
%%                                   {1ex}% afterskip
%                                   {\large \bfseries \raggedright}}
% \renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {.5ex \@plus .2ex}%
%                                      {\normalsize \bfseries \raggedright}}
% \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-2ex\@plus -1ex \@minus -.2ex}%
%                                      {1ex \@plus .2ex}%
%                                      {\normalfont\fontsize{11pt}{12pt}\selectfont\itshape}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}

%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}% 
%  {.5em}%
%  {-1em}%
%  {\normalfont\normalsize\bfseries\parskip=0pt}}
%\setlength\partopsep{0\p@}
%\setlength\parskip{0\p@ \@plus \p@}

%\makeatother
%\parindent=9pt





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "doa"
%%% End:

